Operational Proto-Introspection in Looped Language Models: Reading Correctness Before the Answer

Can one tell, while a language model reasons, whether its answer will be right? Looped models are a good place to ask: they run the same layers several times per token, leaving one hidden state per loop for a probe to read. I probe Ouro-RLTT, a 2.6B-parameter looped model, for what these states reveal about how its reasoning will end. I call such information operational proto-introspection: operational because it is defined by what a probe can read, and proto because nothing here shows that the model itself uses it. In part, yes. Reading the first 48 tokens of reasoning, from answers that state no answer yet, a probe on the hidden states reaches an AUROC of 0.758 on a synthetic logic task, against 0.515 for token confidence. Question difficulty is a rival explanation: on 1,164 further questions, token confidence plus simple features of the question predict about as well. It is not only difficulty: between two answers to the same question, the probe scores the correct one higher 74% of the time. A fine-tuned language model reading the same tokens does about as well. On GSM8K and on a second checkpoint this within-question test is unresolved. A probe that ranks finished candidate answers is weak at layer 8 on the first loop, much better on the second, and as accurate as the last layers by the third, on four Ouro checkpoints. The direction it reads is largely shared across loops: a probe trained on the last loop reads the first nearly as well as a probe trained there. The signal helps decide what to do with finished outputs. It improves abstention over surface features and picks correct answers among candidates better than chance, though surface features pick about as well. Once several samples are finished, a baseline that knows their agreement leaves the answer-free probe nothing measurable to add. None of my attempts to use it to make the model generate better answers worked.

==> paper_style/boxes.tex <==
\tcbset{
  kirinbase/.style={
    enhanced,
    breakable,
    boxrule=0.55pt,
    arc=2.5mm,
    outer arc=2.5mm,
    left=3.2mm,right=3.2mm,top=2.4mm,bottom=2.4mm,
    before skip=6pt,after skip=7pt,
    fonttitle=\sffamily\bfseries,
    coltitle=KirinInk,
    coltext=KirinInk
  }
}

\newtcolorbox{abstractbox}{
  kirinbase,
  title=Abstract,
  colback=white,
  colbacktitle=white,
  coltitle=KirinAccentDark,
  colframe=KirinAccent,
  borderline north={1.0pt}{0pt}{KirinAccent},
  fontupper=\small,
  before upper={\setlength{\parindent}{1em}}
}

% Companion to abstractbox for the page-2 "Results at a glance" layer: same
% framing, no title — the section heading inside the box carries the name.
\newtcolorbox{glancebox}{
  kirinbase,
  colback=white,
  colframe=KirinAccent,
  borderline north={1.0pt}{0pt}{KirinAccent},
  fontupper=\small,
  before upper={\setlength{\parindent}{1em}}
}

\newtcolorbox{resultbox}[1][Result]{
  kirinbase,title=#1,
  colback=KirinAccentFaint,
  colbacktitle=KirinAccentPale,
  coltitle=KirinAccentDark,
  colframe=KirinAccent,
  borderline west={2.2pt}{0pt}{KirinAccent}
}

\newtcolorbox{scopebox}[1][]{
  kirinbase,
  title=#1,
  colback=KirinAccentFaint,
  colframe=KirinRule,
  borderline west={1.6pt}{0pt}{KirinAccent},
  fontupper=\small
}

\newtcolorbox{auditbox}[1][Audit note]{
  kirinbase,title=#1,
  colback=KirinAccentFaint,
  colbacktitle=KirinAccentPale,
  coltitle=KirinUnresolved,
  colframe=KirinUnresolved,
  borderline west={2.2pt}{0pt}{KirinUnresolved}
}

\newtcolorbox{roadmapbox}[1][How to read this paper]{
  kirinbase,title=#1,
  colback=white,
  colbacktitle=white,
  coltitle=KirinAccentDark,
  colframe=KirinRule,
  borderline north={1.0pt}{0pt}{KirinAccent},
  fontupper=\small
}

% Pandoc block quotes become restrained scope/proposition boxes.
\renewenvironment{quote}{\begin{scopebox}}{\end{scopebox}}


==> paper_style/palette.tex <==
\definecolor{KirinInk}{HTML}{172027}
\definecolor{KirinMuted}{HTML}{52606A}
\definecolor{KirinRule}{HTML}{D6DDE1}
\definecolor{KirinBaseline}{HTML}{7D858C}
\definecolor{KirinPositive}{HTML}{16756A}
\definecolor{KirinUnresolved}{HTML}{8F6400}
\definecolor{KirinNegative}{HTML}{A94442}
\definecolor{KirinLink}{HTML}{2E4A75}

\ifkirinmethodology
  \definecolor{KirinAccent}{HTML}{B85C1E}
  \definecolor{KirinAccentDark}{HTML}{874319}
  \definecolor{KirinAccentPale}{HTML}{FBF0E6}
  \definecolor{KirinAccentFaint}{HTML}{FDF8F3}
\else
  \definecolor{KirinAccent}{HTML}{3A5683}
  \definecolor{KirinAccentDark}{HTML}{263C63}
  \definecolor{KirinAccentPale}{HTML}{EDF1F7}
  \definecolor{KirinAccentFaint}{HTML}{F7F9FC}
\fi
\color{KirinInk}



==> paper_style/tables.tex <==
\sisetup{
  detect-all,
  input-open-uncertainty=,
  input-close-uncertainty=,
  table-number-alignment=center,
  group-separator={,},
  group-minimum-digits=4
}

\setlength{\tabcolsep}{4.5pt}
\renewcommand{\arraystretch}{1.12}
\arrayrulecolor{KirinRule}
\AtBeginEnvironment{longtable}{%
  \small
  \setlength{\tabcolsep}{4pt}%
  \renewcommand{\arraystretch}{1.10}%
}
\AtBeginEnvironment{tabular}{\small}
\setlength{\LTpre}{5pt}
\setlength{\LTpost}{6pt}
\setlength{\heavyrulewidth}{0.8pt}
\setlength{\lightrulewidth}{0.45pt}
\setlength{\cmidrulewidth}{0.35pt}
\newcommand{\kirintablehead}[1]{\rowcolor{KirinAccentPale}\sffamily\bfseries #1}
\newcommand{\statusEstablished}{\textsc{Established}}
\newcommand{\statusBounded}{\textsc{Bounded screen}}
\newcommand{\statusUnresolved}{\textsc{Unresolved}}
\newcommand{\statusDiagnostic}{\textsc{Diagnostic}}
\newcommand{\statusRetracted}{\textsc{Retracted}}
\newcommand{\statusHistorical}{\textsc{Historical}}
\newcommand{\statusCorrected}{\textsc{Corrected}}



==> paper_style/titlepage.tex <==
\newcommand{\KirinTitleBlock}[7]{%
  \thispagestyle{fancy}%
  \begingroup
  \setlength{\parindent}{0pt}%
  \noindent\begin{minipage}[t]{0.72\linewidth}
    {\sffamily\bfseries\fontsize{8.5pt}{10pt}\selectfont\color{KirinAccent}\MakeUppercase{#1}}
  \end{minipage}%
  \begin{minipage}[t]{0.28\linewidth}
    \raggedleft{\sffamily\fontsize{8.5pt}{10pt}\selectfont\color{KirinMuted}#6}
  \end{minipage}\par
  \vspace{4pt}\color{KirinAccent}\hrule height 0.85pt\color{KirinInk}\vspace{9pt}
  {\sffamily\bfseries\fontsize{23pt}{25.2pt}\selectfont\raggedright #2\par}
  \vspace{4pt}
  {\sffamily\fontsize{15.2pt}{17.5pt}\selectfont\color{KirinAccentDark}\raggedright #3\par}
  \vspace{8pt}\color{KirinRule}\hrule height 0.45pt\color{KirinInk}\vspace{7pt}
  {\sffamily\bfseries\fontsize{11.5pt}{13.2pt}\selectfont #4}\par
  \vspace{2pt}
  {\sffamily\fontsize{8.9pt}{10.6pt}\selectfont\color{KirinMuted}%
    \href{https://github.com/VykosMolt}{github.com/VykosMolt}%
    \enspace\textcolor{KirinRule}{|}\enspace
    \href{https://github.com/VykosMolt/Branching-Looped-Transformer}{github.com/VykosMolt/Branching-Looped-Transformer}%
    \ifstrempty{#5}{}{\enspace\textcolor{KirinRule}{|}\enspace #5}%
  }\par
  \ifstrempty{#7}{}{\vspace{5pt}{\sffamily\fontsize{8.5pt}{10.2pt}\selectfont\color{KirinMuted}#7\par}}
  \vspace{6pt}
  \endgroup
}

\newenvironment{kirinacknowledgment}{%
  \par\vspace{1pt}\begingroup\small\setlength{\parindent}{0pt}%
  \noindent\textbf{Acknowledgments.}\enspace
}{%
  \par\endgroup\vspace{4pt}%
}

